Budgeted Steiner Networks: Three Terminals with Equal Path Weights

Given a set of terminals in 2D/3D, the network with the shortest total length that connects all terminals is a Steiner tree. On the other hand, with enough budget, every terminal can be connected to every other terminals via a straight edge, yielding a complete graph over all terminals. In this work, we study a generalization of Steiner trees asking what happens in between these two extremes. Focusing on three terminals with equal pairwise path weights, we characterize the full evolutionary pathway between the Steiner tree and the complete graph, which contains intriguing intermediate structures.

==> texs/0x-one-d.tex <==
In one dimension, \bsn degenerates; there is no difference between the Euclidean 
and discrete \bsn formulations. 
%
Specifically, no intermediate nodes is needed to connect a pair of terminal 
nodes in 1D. As such, any connections in the Euclidean case corresponds to an 
edge in a connected graph in the discrete setting. 
%
The difference between obstacle-free and obstacle-laden Euclidean \bsn is also 
limited: $m$ obstacles simply partition a \bsn into up to $(m+1)$ \bsns sharing 
the same budget. Therefore, here, we focus on 1D Euclidean \bsn and then 
briefly examine the case with obstacles. 

For a 1D Euclidean \bsn, without loss of generality, assume $L$ is an integer
and all terminals are located at integer coordinates, i.e., for each pair of 
terminal nodes $1 \le i, j \le n$, $d^*_{ij}$, the actual distance between 
$v_i$ and $v_j$, is an integer and $d^*_{1n} = d^*$. The problem is only 
meaningful when $d \ge L$. 
%
We provide a dynamic programming (DP) routine for minimizing Eq.~\eqref{eq:obj} 
that runs in time polynomial with respect to $n$ and $L$, which yields a 
pseudo-polynomial time algorithm overall. 
%
The DP routine will recursively build a function 

$$
f(\ell, i, j) := J^*_{ij}(\ell) = \min \sum_{i \le i' < j' \le j} w_{i'j'}d_{i'j'},
$$
where a budget of $\ell$ is allocated to connect terminals between $v_i$ and 
$v_j$, $1 \le i \le j \le n$, inclusive. To compute $J^*(L) = f(L, 1, n)$, we 
can use DP to build $f(\ell, \cdot, \cdot)$ starting from $\ell = 1$ until 
$\ell = L$, the actual allocated budget. 

Before describing the DP recursion, we make the observation that for 
$f(\ell, i, j)$, if $\ell \ge d^*_{ij}$, then $f(\ell, i, j) = \sum_{i \le i' 
< j' \le j} w_{i'j'}d^*_{i'j'}$ is at the minimum, fixed, and trivial to 
compute. Therefore, $f(\ell, i, j)$ is only not trivial to compute when 
$\ell < d^*_{ij}$. When this is the case, there must be a terminal node 
$i < k < j$ where $k$ is not connected to terminals on the left or terminals 
on the right (possibly both). In other words, we may compute $f(\ell, i, j)$ 
via the recursion

$$
f(\ell, i, j) =\left\{\begin{array}{ll}
\displaystyle\sum_{i \le i' < j' \le j} w_{i'j'}d^*_{i'j'} & \ell = d^*_{ij} \\
&\\
\displaystyle\min_{
\begin{scriptsize}
\begin{array}{c}\ell' + \ell'' = \ell\\ i < k < j
\end{array}
\end{scriptsize}} [f(\ell', i, k)  + f(\ell'', k, j)]
& \ell < d^*_{ij}
\end{array}  \right.
$$

For computing $f(\ell, 1, n)$, the recursion needs to check about $n\ell$ 
different sums. This leads to an $O(nL^2)$ algorithm for computing 
$J^*(L) = f(L, 1, n)$. The recursion applies to 1D Euclidean \bsn with 
obstacles without modification, though it is clear that using obstacle 
information can reduce the amount of computation. 
\textcolor{red}{Mention that scaling based method might help with the 
computation? We don't need to actually perform any analysis.}

In the special case where $w_{ij} = 1$ for all $1 \le i \le j \le n$, 
$f(L, 1, n)$ is minimized when the number of pairwise connections between 
terminals is maximized. 

